Generating Persuasive Responses to Customer Reviews with Multi-Source Prior Knowledge in E-commerce

Customer reviews usually contain much information about one's online shopping experience. While positive reviews are beneficial to the stores, negative ones will largely influence consumers' decision and may lead to a decline in sales. Therefore, it is of vital importance to carefully and persuasively reply to each negative review and minimize its disadvantageous effect. Recent studies consider leveraging generation models to help the sellers respond. However, this problem is not well-addressed as the reviews may contain multiple aspects of issues which should be resolved accordingly and persuasively. In this work, we propose a Multi-Source Multi-Aspect Attentive Generation model for persuasive response generation. Various sources of information are appropriately obtained and leveraged by the proposed model for generating more informative and persuasive responses. A multi-aspect attentive network is proposed to automatically attend to different aspects in a review and ensure most of the issues are tackled. Extensive experiments on two real-world datasets, demonstrate that our approach outperforms the state-of-the-art methods and online tests prove that our deployed system significantly enhances the efficiency of the stores' dealing with negative reviews.

==> backup/backup.tex <==
% %%
% %% This is file `sample-sigconf.tex',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% samples.dtx  (with options: `sigconf')
% %% 
% %% IMPORTANT NOTICE:
% %% 
% %% For the copyright see the source file.
% %% 
% %% Any modified versions of this file must be renamed
% %% with new filenames distinct from sample-sigconf.tex.
% %% 
% %% For distribution of the original source see the terms
% %% for copying and modification in the file samples.dtx.
% %% 
% %% This generated file may be distributed as long as the
% %% original source files, as listed above, are part of the
% %% same distribution. (The sources need not necessarily be
% %% in the same archive or directory.)
% %%
% %% The first command in your LaTeX source must be the \documentclass command.
% \documentclass[sigconf]{acmart}
% %% NOTE that a single column version is required for 
% %% submission and peer review. This can be done by changing
% %% the \doucmentclass[...]{acmart} in this template to 
% %% \documentclass[manuscript,screen]{acmart}
% %% 
% %% To ensure 100% compatibility, please check the white list of
% %% approved LaTeX packages to be used with the Master Article Template at
% %% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
% %% before creating your document. The white list page provides 
% %% information on how to submit additional LaTeX packages for 
% %% review and adoption.
% %% Fonts used in the template cannot be substituted; margin 
% %% adjustments are not allowed.

% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% % \setcopyright{acmcopyright}
% % \copyrightyear{2018}
% % \acmYear{2018}
% % \acmDOI{10.1145/1122445.1122456}

% \usepackage{booktabs}
% \usepackage{multirow}

% %% These commands are for a PROCEEDINGS abstract or paper.
% % \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% % \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection, June 03--05, 2018, Woodstock, NY}
% % \acmPrice{15.00}
% % \acmISBN{978-1-4503-XXXX-X/18/06}

% % \acmSubmissionID{669}

% \setcopyright{acmcopyright}
% \copyrightyear{2021}
% \acmYear{2021}

% \acmConference[CIKM '21]{The 30th ACM International Conference on Information and Knowledge Management}{November 1--5, 2021}{Online}
% \acmBooktitle{The 30th ACM International Conference on Information and Knowledge Management (CIKM '21), November 1--5, 2021, Online}
% \acmPrice{15.00}



% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}

% %%
% %% end of the preamble, start of the body of the document source.
% \begin{document}

% %%
% %% The "title" command has an optional parameter,
% %% allowing the author to define a "short title" to be used in page headers.
% % \title{Persuasive Response Generation to User Review in E-commerce with Multi-Source Textual Knowledge}
% \title{\textcolor{red}{Generating Persuasive Responses to User Reviews with Multi-Source Textual Knowledge in E-commerce}}

% %%
% %% The "author" command and its associated commands are used to define
% %% the authors and their affiliations.
% %% Of note is the shared affiliation of the first two authors, and the
% %% "authornote" and "authornotemark" commands
% %% used to denote shared contribution to the research.
% % \author{anonymous}
% \author{Bo Chen, Guohua Wu, Feng-Lin Li, Xing Gao, Ji Zhang}
% \email{{herbert.cb, guohuawu.wgh, fenglin.lfl, gaoxing.gx, zj122146}@alibaba-inc.com}
% \affiliation{%
%   \institution{Alibaba Group Inc.}
%   \city{Hangzhou}
%   \country{China}
% }

% % \author{Lars Th{\o}rv{\"a}ld}
% % \affiliation{%
% %   \institution{The Th{\o}rv{\"a}ld Group}
% %   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
% %   \city{Hekla}
% %   \country{Iceland}}
% % \email{larst@affiliation.org}

% % \author{Valerie B\'eranger}
% % \affiliation{%
% %   \institution{Inria Paris-Rocquencourt}
% %   \city{Rocquencourt}
% %   \country{France}
% % }

% % \author{Aparna Patel}
% % \affiliation{%
% %  \institution{Rajiv Gandhi University}
% %  \streetaddress{Rono-Hills}
% %  \city{Doimukh}
% %  \state{Arunachal Pradesh}
% %  \country{India}}

% % \author{Huifen Chan}
% % \affiliation{%
% %   \institution{Tsinghua University}
% %   \streetaddress{30 Shuangqing Rd}
% %   \city{Haidian Qu}
% %   \state{Beijing Shi}
% %   \country{China}}


% % %%
% % %% By default, the full list of authors will be used in the page
% % %% headers. Often, this list is too long, and will overlap
% % %% other information printed in the page headers. This command allows
% % %% the author to define a more concise list
% % %% of authors' names for this purpose.


% %%
% %% The abstract is a short summary of the work to be presented in the
% %% article.
% \begin{abstract}
% %   In E-commerce, user experience of products is mainly conveyed through reviews, However, negative reviews will greatly affect the sellers’ revenue and other buyers' purchase behaviors. An unpersuasive review response often fails to change the impression of the product on the other buyers. Therefore, making a persuasive response to negative reviews is an important behavior for sellers, which is time-consuming and professional yet. Past researches used sequence-to-sequence generation algorithms to produce review response. Their research often focused on a limited number of information sources such as product attributes, and it was easy to generate general responses. They also ignored the multi-aspect related issues in the generation of persuasive responses. In this work, we first defined persuasive response and constructed a relevant dataset TAOBAO MAKEUP to provide a solid foundation for future research, and proposed a Multi-Source Encoder to encode different textual knowledge such as product titles, seller names, product attributes, and historical (review, response) pairs, which provide the source of persuasiveness. In addition, in order to alleviate multi-aspect related issues, we propose a hierarchical attention mechanism to model the attention to different aspect in the response generation stage. Our proposed algorithm not only significantly surpasses the existing SOTA text generation model on the currently public dataset TAOBAO CLOTHES\cite{zhao2019review}, but also brings 6.01 BLEU absolute improvement on TAOBAO MAKEUP comparing with the pre-trained baseline.

% \textcolor{red}{User review is an important way to express user experiences in E-commerce. In general, while positive reviews are beneficial to sellers, negative ones will largely influence other consumers and may lead to decline in sales. To reduce the disadvantageous effect, it is necessary to carefully and persuasively reply to each negative review. Existing sequence-to-sequence generation methods often use limited information sources that may result in general responses, and fail to respond to some mentioned and important aspects in a review (i.e., the multi-aspect issue). In this work, we first define what persuasive response is and accordingly construct a TAOBAO MAKEUP dataset. To provide rich information, we propose a multi-source Encoder to encode different kinds of textual knowledge such as product titles, seller names, product attributes, and historical manually written (review,response) pairs. To alleviate the multi-aspect issue, we propose a hierarchical attention mechanism to model the attention to the different aspects in a review during response generation. Our approach not only significantly outperforms the existing SOTA text generation model on the public TAOBAO CLOTHES dataset, but also brings an absolute improvement of 6.01 in BLEU on our TAOBAO MAKEUP dataset.}
% \end{abstract}

% % \cite{zhao2019review}
% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10010147.10010178.10010179.10010182</concept_id>
% <concept_desc>Computing methodologies~Natural language generation</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computing methodologies~Natural language generation}

% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% \keywords{ natural language processing, natural language generation, E-commerce}

% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% % \begin{teaserfigure}
% %   \includegraphics[width=\textwidth]{sampleteaser}
% %   \caption{Seattle Mariners at Spring Training, 2010.}
% %   \Description{Enjoying the baseball game from the third-base
% %   seats. Ichiro Suzuki preparing to bat.}
% %   \label{fig:teaser}
% % \end{teaserfigure}

% %%
% %% This command processes the author and affiliation and title
% %% information and builds the first part of the formatted document
% \maketitle
% \begin{figure}[!h]
%     \small
%   \centering
%   \includegraphics[width=\linewidth]{showcase_v2.pdf}
%   \caption{A sample of E-commerce (review, response) pair}\label{figure:sample}
%   \Description{The review mentions two aspect in underlined text:(1) awful smell and (2) fake. And the generated response reply to each aspect in underlined text.}
% \end{figure}
% \section{Introduction}

% With the development of E-commerce technology, more and more users prefer to shop on various E-commerce platforms.
% The product reviews are important determinants of customers' purchase decision in online shopping environments, and the content of reviews will heavily influence the business revenue.


% Here, the impact of negative reviews is far greater than that of positive reviews. As the old saying goes, bad news has wings. The present of an organizational response to negative reviews enhance customer inferences of trust and concern\cite{sparks2016responding}. 
% \cite{zhao2019review} also found that sellers who provide high-quality responses often have larger sales volume than those who do not. In addition, unpersuasive responses such as "sorry for the bad experience, we'll do better next time" can't dispel customers' doubts. Therefore, it is an important and frequent behavior for sellers to make persuasive response to the negative user reviews. We observed that a persuasive response to a negative review usually includes the following two characteristics:
% \begin{itemize}
%     \item \textbf{Review Relevance}: Review and response content often correspond point by point, as is shown in Figure 1. There are two vital aspects (1) and (2) underlined in the review, and there are corresponding (1) and (2) points underlined in the response;
%     \item \textbf{Response Professionalism}: Seller usually needs common knowledge or product knowledge to write a persuasive response, and these knowledge can't be obtained from some common used knowledge base like Freebase\cite{bollacker2008freebase} and Wikipedia, as is shown by the red underline in the response in Figure 2;
% \end{itemize}
% In addition, the response is usually related to the seller, and different sellers often have different nick names or response scripts, as is shown in the blue dash line in Figure 1.

% In the past, researchers often used the method of sequence to sequence generation to provide automatic review response\cite{zhao2019review,gao2019automating,gao2020automating}, but their method didn't solve the above problem well. \cite{zhao2019review} first proposed the problem of review response generation, but their method is only evaluated in clothes category. The review types of clothes categories only focus on a few aspect such as "material" and "genuine product", and their method depends on the parametric memory\cite{DBLP:conf/nips/LewisPPPKGKLYR020} of the model, which makes the results tend to be general and cannot be updated in time; \cite{gao2019automating} proposed integrating the meta information of review, such as the category of the app and 
% rating of review, to improve the performance of generation. These features are more effective in app comments rather the E-commerce. In the follow-up work, \cite{gao2020automating} integrate the recall review information, but their method does not pay attention to the multi-aspect correspondence problem widely existed in the responses. \cite{kew2020benchmarking} evaluated several different models on hotel data.

% In order to better solve and explore the above two problems, we first construct the TAOBAO MAKEUP dataset, which contains 100 thousands (reply,response) pairs, 128 sub-category and  mainly bad reviews.
% Different from the previous research, we use all the available textual knowledge as the information sources to solve the two problems existing in the review response generation. This is the first attempt in the field of E-commerce review response generation. The textual knowledge we use includes review, product titles, product attributes, historical review and response pairs, seller name:

% Given a (review, product, seller name) triple, we use ElasticSearch\cite{gormley2015elasticsearch} to get the relevant (review, response) pairs from a pre-constructed (review, response) pool according to the seller name, product title and bad review. Then, a encoder of a pre-trained BART\cite{lewis2020bart} model equipped with a so-called Multi-Source Encoder is used to encode the all the textual knowledge mentioned before. Finally, A BART decoder with Pointer Generator Network and Hierarchical Attention Mechanism(HAM) are used to generate the response according to the textual knowledge. HAM is used to guide the decoder in the generation progress. Compared with the published methods, our proposed method achieves state of the art. In addition, compared with the baseline based on pre-training, our method also brings 5.53 points of BLEU absolute improvement in TAOBAO MAKEUP dataset;

% In general, our contribution has three aspects:
% \begin{itemize}
%     \item The TAOBAO MAKEUP dataset: We first discover and define the meaning of persuasive response . In addition, TAOBAO MAKEUP dataset is constructed to explore this problem. The dataset includes 100k (reviews, seller names, product titles, attributes, recall review pairs) samples, including 100+ sub Category. This dataset provides a solid research foundation for generating persuasive responses.
%     \item The Multi-Source Encoder: We propose the Multi-Source Encoder to encode different textual knowledge such as product titles, seller names, product attributes, and historical (reiview,response) pairs, which provide the source of persuasiveness.
%     \item The hierarchical attention mechanism :A hierarchical attention mechanism is proposed to alleviate the multi-aspect related problem of review response.
% \end{itemize}

% The following sections will be organized as follows:
% The second section introduces preliminaries about the task definition and BART model;
% The third section describes the proposed method; the fourth section introduce the TAOBAO MAKEUP dataset; the fifth section conducts an experimental analysis; The sixth section introduce related works in this area; We make a conclusion at the last section.
% \section{PRELIMINARIES}
% \subsection{Task Definition}
% In this section, we introduce our key notations used in this paper. The input of our model is 
% the review $X$, the product title $T$, the seller name $S$, the product properties $P$ and some (review, response) pairs $R$ recalled by ElasticSearch\cite{gormley2015elasticsearch}. The output of our model is the review response $Y$. The proposed model can be represented as $f:(X,T,S,P,R)->Y$.

% $X = \{x_1, x_2,..., x_n \} $ denotes a review of length $n$, where $x_i$ represents a word. $P=\{(k_1,v_1),(k_2,v_2),...,(k_l,v_l)\}$ represents $l$ properties of the reviewed product, where $k_i$ is the i-th property field and $v_i$ is the corresponding property value. $T = \{t_1, t_2,..., t_u\}$ is the product title of length $u$. $S = \{s_1, s_2,..., s_w\}$ is the seller name of length $w$. $R=\{(f_1,r_1),(f_2,r_2),...,(f_m,r_m)\}$ is the notion of $m$ recalled (review,response) pairs,
% where $f_i$ is a recalled review, while $r_i$ is the corresponding response to the recalled review.  $k_i$, $v_i$, $f_i$, $r_i$ are a sequence of word. $Y = \{y_1, y_2,..., y_v \} $ denotes a target response for review of length $v$. 
% \subsection{BART}
% The seq2seq framework could be modelled using any encoder-decoder. Here we use BART-base\cite{lewis2020bart} as the skeleton, which is commnonly used in many downstream tasks\cite{DBLP:conf/acl/GuLLL16,liu2020multilingual,kumar2020data}. It is a denoising autoencoder
% for pretraining sequence-to-sequence models based on seq2seq transformer\cite{DBLP:conf/nips/VaswaniSPUJGKP17}. Specifically, it is trained by corrupting documents and then optimizing a reconstruction loss—the cross-entropy between the decoder’s output and the original document. 
% The documents corruption method includes Token Masking, Token Deletion, Text Infilling, Sentence Permutation, Document Rotation.
% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth,height=0.5\linewidth]{overview_v2.pdf}
%   \caption{The Overview of the Whole Framework}\label{figure_overview}
%   %\Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure*}
% \section{Method}

% \subsection{Overview}
% As is shown in the Figure \ref{figure_overview}, given a sample (X,T,S,P), we use (X,T,S) to recall (review, response) pairs $R$ from a pre-constructed pool via ElasticSearch\cite{gormley2015elasticsearch} at the first. The purpose of retrieval step is to find corresponding responses of similar review. Then we generate the review related response in a seq2seq fashion, which is a modified BART model.

% The reason of using seller name S and product title T in the retrieval process is to avoid introducing unrelated information from other seller and product. After the retrieval progress, we use a in-house review pair ranking model to rank the $(X,f_i)$ pairs, which help us to get the top $m$ related (review, response) pairs $R$. 
% % The detail about the data construction will be introduced in section \ref{section:da}.

% After the retrieval progress, We encode the $(X,T,S,P,R)$ with the multi-source encoder, which convert the information into a memory matrix. Finally
% with the aid of Hierarchical Attention Mechanism(\textbf{HAM}), a BART decoder with a pointer generator network will generate the response word by word according to the memory matrix.

% \subsection{Multi-Source Encoder}

% Our basic encoder is a pre-trained BART encoder, which has not defined the approach to deal with multi-source information. Thus, the key point here is how to encode and fusion the information from different source. Here, we divide the information sources into two categories: text and text pairs, we encode them with different encoder. The former includes the review $X$, the product title $T$, and seller name $S$, while the latter includes property pairs $P$ and (review, response) pairs $R$. 

% \subsubsection{Text Encoder}\label{subsubsection:textencoder}
% As is shown in Figure \ref{figure_overview}, we use the embedding layer and the first layer of BART encoder as the text encoder. Formally, we concatenate X,T,S with [SEP] symbol as $\hat{X} =\{x_1,x_2,...,x_n,[SEP],t_1,t_2,...,t_u,$
% $[SEP],s_1,
% s_2,...,s_w\}$. The max number of $n,u,w$ are setting to a fixed values, we will truncate sentences that are too long. Text encoder will convert $\hat{X}$ into embedding matrix $\mathbf{\hat{X}}=\{\mathbf{x_1,x_2,...,x_{n+u+w+2}}\}$, assume the hidden size of BART is $D$, then $\hat{\mathbf{X}}\in \mathbb{R}^{(n+u+w+2)\times D}$.

% \subsubsection{Text Pairs Encoder} We encode each pair in properties P and (review, response) pairs R with text pair encoder. 
% Like the operation in the \ref{subsubsection:textencoder}, we first concatenate a text pair with symbol [PAIR] as $P_i=\{p_1,p_2,...p_n,$
% $[PAIR],q_1,q_2,..q_m\}$, then encode P into embedding matrix $\mathbf{P_i}=\{\mathbf{p_1,p_2,...p_n,p_{n+1},p_{n+2},p_{n+3},..,p_{n+m+1}}\}$ with text encoder defined before. After the encoding progress, we use a aggregation function $g(P_i)$ to convert the $P_i$ into a single vector $\mathbf{p_i}$. Here we use the following pooling function to reduce the amount of calculation:
% \begin{equation}
%   g(P)=max\_pool(P)
% \end{equation}
% In this way, we get a fixed dimension vector to represent each text pair. Videlicet, we get a matrix $\hat{\mathbf{P}}\in\mathbb{R}^{l_p\times D}$ to represents $l_p$ properties of a product and a matrix $\hat{\mathbf{R}}\in\mathbb{R}^{m\times D}$ to represents 
% $m$ (review, response) pairs.

% \subsubsection{Multi-Source Fusion}
% to distinguish different source, we add a specific random initialized type embedding vector to each component of the output of text encoder and text pairs encoder as is shown in the Figure. $T(0),T(1),T(2)\in \mathbb{R}^D$ represents for current review, properties and history (review, response) pairs type embedding respectively, the type embedding vector is actually broadcasting to a matrix to support the text length or number of pairs:
% \begin{equation}
%   \overline{\mathbf{X}}=\mathbf{\hat{X}}+ T(0),
%   \overline{\mathbf{P}}=\mathbf{\hat{P}}+ T(1),
%   \overline{\mathbf{R}}=\mathbf{\hat{R}}+ T(2)
% \end{equation}
% Then we concatenate the three matrix
% \begin{equation}
%     \mathbf{M}=[\mathbf{\overline{X}:\overline{P}:\overline{R}}] \in \mathbb{R}^{(n+u+w+l+m+2)\times D}
% \end{equation}
% We take the $\mathbf{M}$ as the input of the remain layers of BART encoder except the first layer. We mark the output of the encoder as $\mathbf{M}^{(n_{l})}$, where $n_l$ is the number of BART encoder layers. 
% \begin{equation}
%     \mathbf{M}^{(n_{i+1})}=BART\_ENCODE\_LAYER(\mathbf{M}^{(n_{i})})
% \end{equation}

% \subsection{Hierarchical Attention Mechanism}
% As is shown in Figure \ref{figure:sample},
% reviews often have multiple aspects, and experts usually write responses to each aspect one by one. To model this situation, we design a Hierarchical Attention Mechanism(HAM) in the decoding progress. We insert a special token [SENT] after every semantic fragment in the review part. These semantic fragments are separated by punctuation marks such as comma, period, and exclamation mark.

% A review like \textit{"It’s oily after putting it on for at most two hours, and it smells weird."} will be convert into \textit{"[SENT] It’s oily after putting it on for at most two hours\textbf{,} [SENT] and it smells weird\textbf{.} "}. Denote the indexes of 
% [SENT] in M as set $I_s=\{s_1,s_2...,s_m\}$, we first gather the vectors corresponding to $I_s$ in $M^{(n_{l})}$ as a Matrix $M_s$:
% \begin{equation}
%     M_s=[(h_{s_1}^e)^T:(h_{s_2}^e)^T:...:(h_{s_m}^e)^T],s_i \in I_s 
% \end{equation}
% Here $h_i^e$ is the i-th row vector of encoder output matrix $M^{(n_{l})}$.
% Denote $h_t \in \mathbb{R}^{D}$ as the last hidden layer of current decoding time step of BART decoder, HAM will first calculate a attention vector $a_{t}$ over $M_s$ via $h_t$:
% \begin{equation}
% \begin{aligned}
%     e_{t,i}=& w_1^T*tanh(W_1*(h^e_{s_i})^T+W_2*h_t+b_1)\\
%     \lambda_{t,i}=&\frac{exp(e_{t,i})}{\sum\limits_{s_k \in I_s}exp(e_{t,s_k})}\\
%     a_t=&\sum\limits_{s_i \in I_s} \lambda_{t,i}*h_{s_i}^e
% \end{aligned}
% \end{equation}

% With the attention vector $a_t$ and the hidden states $h_t$, HAM use a two layer neural networks to get the
% vocabulary distribution $P_v(y_t)$ a vocabulary:
% \begin{equation}
% \begin{aligned}
%     P_v(y_t)=softmax(W_5*(W_3*h_t+W_4*a_t+b_2)+b_3)
% \end{aligned}
% \end{equation}
% Here, $W_1,W_2,W_3,W_4 \in \mathbb{R}^{D \times D},b_1,b_2 \in \mathbb{R}^{D\times 1}, W_5 \in \times \mathbb{R}^{D\times |V|},b_3 \in \mathbb{R}^{1\times |V|}$ are learnable parameters.

 
% \subsection{Bart Decoder with PGN}
% The contents in X such as product title, review, seller name are referenced very often in responses text of experts. Based on this observation, we add a Pointer Generator Networks on the BART decoder over the representation of X.

% We treat the first $l_x=n+w+u+2$ rows of $M^{(n_{l})}$ as the representation of X, where $l_x$ is the length of the concatenated information with symbol [SEP]. Formally,
% \begin{equation}
%     X^{n_l}=M^{(n_{l})}[:l_x,:]
% \end{equation}
% Denote $h_t$ as the last hidden layer of current decoding time step of BART decoder, the Pointer Generator will first calculate a attention score $\beta_{t}$ over $X^{n_l}$ via $h_t$:
% \begin{equation}
% \begin{aligned}
%     \alpha_{t,i}=& w_6^T*tanh(W_6*(X^{n_l}_i)^T+W_7*h_t+b_6)\\
%     \beta_{t,i}=&\frac{exp(\alpha_{t,i})}{\sum\limits_{l_x}exp(\alpha_{t,l_x})}\\
% \end{aligned}
% \end{equation}
% As a result, $P_c(y_t)$ is the
% copy distribution over the vocabulary extended by X, defined as 
% \begin{equation}
% \begin{aligned}
%     P_c(y_t)=\sum_{i:x_i=y_t}\beta_{t,i}
% \end{aligned}
% \end{equation}
% The final probability $P(y_t)$ of generating
% word $y_t$ is defined as a mixture of the extended
% vocabulary distribution $P_v(y_t)$ and the copy distribution $P_c(y_t)$\footnote{The formula is different from the original pointer generator network, we don't find the difference in performance between this two method}:
% \begin{equation}
% \begin{aligned}
%     P(y_t)=&\epsilon*P_v(y_t)+(1-\epsilon)*P_c(y_t)\\
%     \epsilon=&sigmoid(w_{\epsilon}^T*h_t+b_{\epsilon})
% \end{aligned}
% \end{equation}
% Here, $W_6,W_7 \in \mathbb{R}^{D \times D},b_6 \in \mathbb{R}^{D\times 1}, W_5 \in \times \mathbb{R}^{D\times |V|},b_{\epsilon} \in \mathbb{R},w_{\epsilon} \in \mathbb{R}^{D \times 1}$ are learnable parameters.
% We optimize the whole model with object function:
% \begin{equation}
% \begin{aligned}
%     L(\theta;(\mathcal{X},\mathcal{Y}))=-\sum\limits_{(X,T,S,P,R) \in \mathcal{X},
%     Y \in \mathcal{Y}}\sum\limits_{y_t \in Y}log(P(y_t))
% \end{aligned}
% \end{equation}

% \section{the TAOBAO MAKEUP Dataset}

% \subsection{Dataset Construction}\label{section:da}
% We collect the data of the TAOBAO MAKEUP dataset from taobao.com, one of the largest online
% shopping website in China. There are 100K (review, product properties, seller name, commodity title, recalled response pairs,
% response) in the corpus which all belong to the
% category of Makeup.  The makeup is a parent category which contains almost 100+ sub-category vary from cleansing, nose cream to false eyelashes. Due to the sub-category variety, the negative review is much more hard to response than the TAOBAO CLOTHES dataset for a single person. Here, we drop the data with good sentiment via a in-house review sentiment classification tool.

% The properties is collected from the
% product page in the website. We also build a elastic search index based on a more huge dataset, which is used as the recall pool of the (review, response) pairs. The search scope of a single query is limited to the same seller name and sub-category id. And we treat the review with 2.0 boosting weight, while the commodity title is given 1.0 boosting weight. The recalled (review, response) pairs is ranked by a in-house review pair ranking model 
% which yield 0.509 f1 in the corresponding test set.
% \begin{table*}[!htbp]
% \begin{tabular}{@{}llcc@{}}
% \toprule
%                                                                                                  &                                        & Tabao Cloth          & TAOBAO MAKEUP        \\ \midrule
% \multirow{3}{*}{\#num}                                                                           & \multicolumn{1}{l|}{train}             & 80000                & 104532               \\
%                                                                                                  & \multicolumn{1}{l|}{valid}             & 10000                & 2986                 \\
%                                                                                                  & \multicolumn{1}{l|}{test}              & 10000                & 14054                \\ \midrule
% \multirow{2}{*}{overview}                                                                        & \multicolumn{1}{l|}{negative/positive} & 70\%:30\%            & 100\%:0\%            \\
%                                                                                                  & \multicolumn{1}{l|}{\#category}        & -                    & 128                  \\ \midrule
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}relevance\\ (r/p/f1)\end{tabular}}                    & \multicolumn{1}{l|}{title}             & -                    & 0.0443/0.1541/0.0668 \\
%                                                                                                  & \multicolumn{1}{l|}{property}          & 0.0204/0.0233/0.0204 & 0.0589/0.0648/0.0561 \\
%                                                                                                  & \multicolumn{1}{l|}{recalled\_response}   & -                    & 0.7955/0.3261/0.4375 \\ \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}length(l) \\ or num(n) \\ (min/avg/max)\end{tabular}} & \multicolumn{1}{l|}{title(l)}          & -                    & 4/33.1/61            \\
%                                                                                                  & \multicolumn{1}{l|}{properties(n)}     & 1/14.2/26            & 1/10.6/21            \\
%                                                                                                  & \multicolumn{1}{l|}{response(l)}          & 23/117.8/415         & 18/131.1/562         \\
%                                                                                                  & \multicolumn{1}{l|}{review(l)}       & 19/61.6/360          & 1/32.0/665           \\ \bottomrule
% \end{tabular}
% \end{table*}
% \subsection{Dataset Statistics}
% The basic statistics of the TAOBAO MAKEUP dataset is shown in the table . Different from TAOBAO CLOTHES, our dataset contains 128 sub-category and mainly bad review. We added the title field as one of the sources of generation, which is not shown in the TAOBAO CLOTHES dataset\footnote{Because the published time of the TAOBAO CLOTHES dataset is too early, we couldn't find the matched title and recalled response}. We calculate the relevance score of a sample i based on the formula:
% \begin{equation}
% \begin{aligned}
%     r_i=&\frac{|H_i \cap R_i|}{|R_i|}\\
%     p_i=&\frac{|H_i \cap R_i|}{|H_i|}\\
%     f1_i=&\frac{2*p_i*r_i}{p_i+r_i}\\
% \end{aligned}
% \end{equation}
% Here $H_i$ is the word set of different source such as title or property. $R_i$ is the word set of the corresponding response. We tokenized the word with Jieba\footnote{https://github.com/fxsjy/jieba}.
% Then we use the average $p_i/r_i/f1_i$ over $\mathcal{X}$ in training set as the relevance measurement:
% \begin{equation}
%      p=\frac{\sum_i p_i}{|\mathcal{X}|},
%     r=\frac{\sum_i r_i}{|\mathcal{X}|},
%     f1=\frac{\sum_i f1_i}{|\mathcal{X}|}
% \end{equation}

% As we can see, the relevance scores of recall responses are significantly higher than other sources. And the title relevance $r$ is much more higher than properties, because the length of title is more shorter and title is often more brief. 

% \section{Experiments}
% \subsection{Datasets}
% \subsubsection{TAOBAO CLOTHES}
% The TAOBAO CLOTHES dataset is proposed by \cite{zhao2019review}, which focus on the clothes category and have 80000/10000/10000 for train/valid/test. It's a generally used benchmark in this area.
% \subsubsection{TAOBAO MAKEUP}
% The TAOBAO MAKEUP dataset is collected by us. The detail about the dataset can be found in section \ref{section:da}
% \subsection{Evaluation Metrics}
% \subsubsection{Automatic evaluation Metrics}
% Like \cite{zhao2019review}, we also use BLEU, rouge as the evaluation metric. In addition, we have added a distinct\cite{li2016diversity} indicator to evaluate the repetitive generation in a sentence. Here we use character-granular word segmentation to evaluate sentences to avoid the influence of bad tokenizer.
% \begin{itemize}
% \item {\verb|BLEU|}: BLEU is widely used in neural machine translation and other text generation task with parallel corpus.
% It measures word overlap between the generated text and the ground-truth. As \cite{zhao2019review}, we calculate the BLEU score with NLTK toolkit\footnote{https://www.nltk.org}. 
% \item {\verb|Rouge|}: ROUGE is also a widely used evaluation
% metric in text generation. We report ROUGE- 1, ROUGE-2 and ROUGE-L in this paper.
% \item {\verb|Distinct|}:The distinct score is first proposed by \cite{li2016diversity}, which is used to measure a variety of a corpus. Unlike \cite{zhao2019review}, we don't calculate the distinct score in corpus level. we calculate the distinct score in sentence level to detect repetitive in a sentence.
% \end{itemize}
% \subsubsection{Persuasiveness Evaluation Metric}
% To evaluate the persuasiveness of different method,
% we also conduct human evaluation in this work like \cite{zhao2019review}. We randomly sampled 500 cases and
% invited three volunteers to evaluate the generated responses
% of different models. For each sample (review, seller name,product title,response), volunteers are asked to give a score from
% {1,2,3,4,5}, which represents the quality of response:
% \begin{itemize}
%     \item 1 means
% the response is irrelevant or disfluent with grammatical errors or repetitive;
% \item 2 means the sentence is fluent and grammatically correct, but has nothing to do with the review;
% \item 3 means that the sentence is fluent and grammatically correct, and is related to the comment, but lacks persuasiveness. It is a general reply
% \item 4 indicates that the response is smooth, relevant to review and persuasive, but missing part of aspect appear in the review.
% \item 5 indicates that the response is not only fluent, relevant to the comment, persuasive, and it fully answers every point of the review.
% \end{itemize} 
% \subsection{Compared Method}
% We  compare  the  proposed  method  with  a state of the art E-commerce review response generation baseline and construct several BART-based baseline.
% \begin{itemize}
%     \item {EPI}:EPI\cite{zhao2019review} is the state of the art E-commerce review response generation method which use a additional encoder for product properties, we get the result with their code.
%     \item {BART(baike)}: We use Baidu Encyclopedia data(9.6GB, 9.58 million sentences) to pre-train a BART model in the pretraining fashion, which treat the transformer as a sequence to sequence denoise auto-encoder. Then we concatenate the properties with a [PAIR] symbol and concatenate different sources with [SEP] symbol as the input. The training processing is the same as other method. We drop the title information in this method to make a fair comparsion with EPI.
%     \item {BART(review)}: We use (review, title,seller name, response) quadruples to pre-train a BART model in a supervised fashion. The corpus contains 8.35 million quadruples. We add a type embedding for each source in the embedding layer and use the concatenation way mentioned in BART(baike). \footnote{Due to the data collection time, the pretrain corpus has no overlap with TAOBAO CLOTHES and TAOBAO MAKEUP test/valid set.} After pretraining, we finetune the model on the TAOBAO CLOTHES and TAOBAO MAKEUP seperately. The only difference between BART(baike) and BART(review) is the pretrain method.
%     \item {$retrieval_{top1}$}:The retrieval system mentioned in \ref{section:da} is used as a retrieval baseline. The system is used to rank the review pairs.
%     % \item {$retrieval_{upbound}$}:We use this method to evaluate the up-bound of the retrieval method. We calculate the rouge score between (response,recalled response) pairs $(Y,r_i)$. And we treat the $r_i$ with max rouge scores as the prediction of this method to $Y$, which is hard to achieve due to the missing of $Y$ in real time. 
%     \item {MSE-HAM}: Multi-Source-Encoder(\textbf{MSE}) with the Hierarchical Attention Mechanism(\textbf{HAM}) is the proposed model in this work, we denote the version without 
%   Hierarchical Attention Mechanism as \textbf{MSE}. For TAOBAO CLOTHES dataset, we don't have recall (review, response) pairs P and product title T.
%     % \item {\verb|MSE-HAM|}: 
% \end{itemize}
% \subsection{Hyper Parameters}
% % \begin{table}[h]
% % \caption{Hyper parameters}\label{table:hyp}
% % \begin{tabular}{|l|l|}
% % \hline
% % $n_l$    & 6         \\ \hline
% % D        & 768       \\ \hline
% % $\delta$ & 1e-4/5e-5 \\ \hline
% % $\gamma$ & 0.075     \\ \hline
% % $B$      & 10/20     \\ \hline
% % $n_B$    & 10        \\ \hline
% % \end{tabular}
% % \end{table}
% For EPI, we used the same setting reported in \cite{zhao2019review}. We optimize the other model via Adam optimizer
% %\footnote{These model are implemented in pytorch, we will release the code and the dataset after this work is accepted}.
% Because the expensive time cost of inference, we use the teacher forcing training paradigm\cite{williams1989learning} and use the acc in token level as the basis for early stopping. All models are trained with 10 epochs. The whole hyper parameter includes number of BART hidden layers $n_l=6$, the dimention of hidden layer $D=768$, learning rate $\delta=1e-4/5e-5$\footnote{We found for MSE(-HAM), it's better to use 1e-4 to get a better convergence curve due to different input layers, while we didn't find the improvement of BART in this learning rate}, the warm up\cite{he2016deep} rate $\gamma=0.075$, batch size $B=20$, the number of beam in generation progress $n_B=3$, the max number $m$ of the recalled (review, response) pairs, other hyper parameter about BART can be found in \cite{lewis2020bart}\footnote{We use the codebase of huggingface\cite{wolf2019huggingface}, their configuration can be found in  https://huggingface.co/facebook/bart-base/blob/main/config.json}. 

% % \subsection{Performance comparison and analysis}
% \begin{table*}[]
% \caption{Comparison with different models via various automatic evaluation metrics}\label{table:automatic_eval}
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
%                                     & \multicolumn{5}{c}{TAOBAO CLOTHES}                                                            & \multicolumn{5}{c}{TAOBAO MAKEUP}                                                                                                                           \\ \cmidrule(l){2-11} 
%                                     & bleu           & r-1            & r-2            & r-l            & dis-1/2/3/4             & bleu                      & r-1                       & r-2                       & r-l                       & dis-1/2/3/4                                 \\ \midrule
% \multicolumn{1}{l|}{EPI}            & 15.61          & 36.71          & 18.07          & 28.84          & 0.623/0.809/0.848/0.856 & 12.42                     & 30.39                     & 15.36                     & 27.86                     & 0.494/0.624/0.658/0.664                     \\ \midrule
% \multicolumn{1}{l|}{BART(baike)}    & 12.40          & 34.89          & 14.77          & 24.95          & 0.683/0.887/0.932/0.940 & 28.29                     & 45.61                     & 29.35                     & 39.29                     & 0.692/0.888/0.927/0.935                     \\
% \multicolumn{1}{l|}{BART(review)}   & 16.86          & 38.64          & 18.98          & 28.68          & 0.691/0.898/0.939/0.944 & 33.62                     & 50.66                     & 35.39                     & 44.83                     & 0.705/0.905/0.941/0.945                     \\
% %%\multicolumn{1}{l|}{\quad+PGN}   & 23.08          & 42.68          & 24.43          & 33.78          & 0.691/0.897/0.937/0.941 & 33.92                     & 50.66                     & 35.52                     & 44.95                     & 0.703/0.902/0.939/0.943                     \\
% % \multicolumn{1}{l|}{\quad+PGN}   & -         & -          & -         & -          & - & 38.51                     & 54.52                     & 40.39                     &  49.25                   & 0.710/0.911/0.946/0.950                    \\
% \midrule
% \multicolumn{1}{l|}{retrievel top1} & -              & -              & -              & -              & -                       & 43.61                    & 54.74                   & 41.26	                    & 49.29                    & 0.698/0.906/0.942/0.947\\
% % \multicolumn{1}{l|}{retrievel upbound} & -              & -              & -              & -              & -                       & \multicolumn{1}{l}{76.40} & \multicolumn{1}{l}{80.69} & \multicolumn{1}{l}{74.95} & \multicolumn{1}{l}{79.17} & \multicolumn{1}{l}{0.703/0.907/0.941/0.946} \\
% \midrule
% \multicolumn{1}{l|}{MSE}            & 21.75          & 41.77          & 23.28          & 32.95          & 0.680/0.885/0.926/0.931 & 39.15                     & 54.83                     & 40.60                     & 49.49                     & 0.709/0.911/0.947/0.951                     \\
% \multicolumn{1}{l|}{MSE-HAM}        & \textbf{24.44} & \textbf{43.64} & \textbf{25.67} & \textbf{34.99} & 0.688/0.895/0.936/0.940 & \textbf{39.63}            & \textbf{54.89}            & \textbf{40.62}            & \textbf{49.56}            & 0.705/0.910/0.947/0.951                     \\ \bottomrule
% \end{tabular}
% \end{table*}
% \subsection{Automatic Evaluation}
% We first discuss the experimental results on the automatic evaluation metric. We show the experimental results in Table \ref{table:automatic_eval}. 
% \begin{table}[]
% \caption{Persuasive evaluation of different method. }\label{table:human}
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
%          & 1       & 2      & 3       & 4      & 5       & $score_{avg}$ \\ \midrule
% EPI      & 66.60\% & 7.02\% & 20.58\% & 1.15\% & 4.66\%  & 1.71          \\
% BART & 5.36\%  & 12.30\% & 30.33\% & 9.26\% & 42.75\% & 3.71          \\
% MSE      & 4.85\%  & 13.09\% & 27.27\% & 10.06\% & 44.73\% & 3.76         \\
% MSE-HAM & 2.88\%	&11.38\%	&32.63\% &	8.13\% &	45.00\% &3.81          \\
% $retrieval_{top1}$ & 3.37\% &	18.89\% &	17.45\% &	14.56\%	&45.73\% &3.80 \\

% HUMAN    & 5.84\%  & 6.04\% & 28.14\% & 4.64\% & 55.34\% & 3.95          \\ \bottomrule
% \end{tabular}
% \end{table}
% First of all, we can find that MSE-HAM achieves the SOTA on the two datasets except for the distinct metric. MSE-HAM far surpasses the EPI on both datasets, which is the best publicly published methods. HAM brings 2.69 points of BLEU improvement on TAOBAO CLOTHES dataset. In addition, we find that the pre-trained model is generally better than the EPI method, but on the TAOBAO CLOTHES data, the BART model pre-trained on the Baidu Encyclopedia is even worse than the EPI. However, we observe that the distinct score of BART is always better than EPI, which indicates that the EPI method actually generates a lot of unreadable repetitive sentences. Human evaluation also supports this conclusion in Table \ref{talbe:human}. The failure of BART(baike) shows that a large model which is not pre-trained on the domain corpus may not be better than the method based on seq2seq in automatic metric. 

% We find that for all BART-based model includes MSE and  MSE-HAM, the results of TAOBAO MAKEUP is much better than TAOBAO CLOTHES. Because the TAOBAO MAKEUP training set is more relevant to the test set than TAOBAO CLOTHES. We find that TAOBAO MAKEUP  are relatively concentrated on seller names, and 91.4\% (1196/1308) of the seller names have appeared in the training set. And this value in TAOBAO CLOTHES is 66.6\% (2988/4481). \footnote{This is caused by the inherent differences between 
% makeup industry and clothes industry.}. 

% On TAOBAO MAKEUP, we compare the result of the in-house review pair ranking models with the generation counterpart. We find that only a simple bert-based matching model is better than BART (review) 9.99 BLEU, but the MSE model which integrates retrieval results achieves 39.15 BLEU score, with the help of HAM, the score reaches 39.63.
% \subsection{Persuasiveness Evaluation}

% The result of persuasiveness evaluation on TAOBAO MAKEUP is shown in Table \ref{table:human}, we show the
% percentage of each score. We also give the human performance in the last row and average score in the last column.

% Observing Table 5, we can find that the HAM mechanism has brought a 0.27\% increase in persuasiveness to MSE (the score of 5). The overall score has reached 3.81, and the artificial result is only 3.95; although in the automatic metric, BART is much worse than MSE peer, the numerical value in persuasiveness is quite different. This is because although the model produces different responses, they are not very different to customers, but this kind of 
% response that does not depend on the seller’s existing responses may have more serious problems, such as the introduction of wrong information and inapposite 
% response. In addition, all generative models perform poorly in terms of relevance, as the score 2 part is significantly lower than the human performance, and they are prone to produce unpersuasive responses (the part with a score 3 is higher than human). But comparing with MSE-HAM, the $retrieval_{top1}$ is worse in relevance due the multi-aspect related problem, it's easy to map a response with extra aspect.  In the end, human only get 55\% response to be persuasive on this task, indicating that there is still a lot of space for optimization in this task.
% \subsection{Ablation Study}
% \subsubsection{Robustness of the model}
% We evaluated the performance of MSE-HAM in the absence of some sources of information.
% \begin{table}[]
% \caption{Performance of removing part of source}\label{tab:remove_source}
% \begin{tabular}{@{}lllll@{}}
% \toprule
%                 & BLEU  & r-1   & r-2   & r-l   \\ \midrule
% MSE-HAM          & 39.63 & 54.89 & 40.62 & 49.56 \\
% \quad-properties     & 39.66 & 54.95	 & 40.71	 & 49.64 \\
% \quad-recalled pairs & 32.21 & 49.54	 & 34.13	 & 43.34 \\ \midrule
% MSE-HAM-SD      & 39.64 & 55.32 & 41.29 & 50.11 \\
% \quad-properties     & 39.40 & 55.15 & 41.07 & 49.90 \\
% \quad-recalled pairs & 38.01 & 53.82 & 39.54 & 48.34 \\ \bottomrule
% \end{tabular}
% \end{table}
% We removed the properties and recalled pairs in the inference phase separately. As is presented in Figure \ref{tab:remove_source}, we can find the absence of recalled pairs will hugely influence the performance of our model, the lack of properties is just the opposite. To alleviate this problem, we explore a training trick so-called Source Dropout(SD), which drops the recalled pairs in the training stage with a 30\% probability. As is shown in the Table  \ref{tab:remove_source}, the trick enhances the robustness when the recalled source 
% is missing.
% \subsubsection{The impact of the number of recalls}
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{recall_num_influ.pdf}
%   \caption{BLEU of Different numbers of recalled Pairs}\label{fig:bleu_transfer}
% \end{figure}
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{relevance.pdf}
%   \caption{Relevance score of Different numbers of recalled Pairs}\label{fig:relevance}
%   %\Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}
% \begin{figure*}[!h]
%   \centering
%   \includegraphics[width=\linewidth]{showcase_new.pdf}
%   \caption{Case study, comparing the two baselines with our model}\label{fig:response}
% \end{figure*}
% We also analyze the impact of different number of recalled (review,response) pairs on the model performance of MSE-HAM, MSE-HAM, MSE-HAM-SD in TAOBAO MAKEUP.
% As can be seen in Figure \ref{fig:bleu_transfer}, with the number of retrieved responses
% increasing from 1 to 19, the BLEU-4 score increases, and when the number of retrieved
% responses is set as 7, MSE-HAM yields the best performance. As is shown in Figure \ref{fig:relevance}, we also calculated the  relevance score ranging from 1 to 19. The trend of BLEU curve is closer to the trend of relevance-r. The decrease of relevance P finally brings a slight decrease in the BLEU curve. This phenomenon shows the robustness of our model to the number of recalls. The Source Dropout trick increases the robustness.

% \subsection{Case Study}

% To compare the generated responses between different models, we
% give a examples on Figure \ref{fig:response}. The case in the left of Figure 5 is a
% negative review and responses generated by our model, while the right part is the English version. The EPI method generates repetitive and unreadable responses. The BART method did not respond to the genuine product problem. MSE also ignores the genuine product problem. And it has a hallucination about a person named 'Lina'. Both manual response and MSE-HAM achieve the perfect persuasive response.
% \section{Related Works}
% \subsection{Seq2Seq Framework}
% There has been quite a bit of research on 
% Text generation based on sequence to sequence framework has been widely studied. \cite{sutskever2014sequence} first introduced the Seq2Seq framework, which encode the source sequence with a encoder and decode the target sequence according to the encoder output. The attention mechanism\cite{bahdanau2014neural} is integrated into seq2seq-based neural machine translation to enhance the ability of capturing long term dependency, which is also widely used in other text generation tasks and made great success\cite{xing2018hierarchical,liu2018table,kiddon2016globally}. \cite{DBLP:conf/nips/VaswaniSPUJGKP17} proposed transformer-based seq2seq framework, based solely on multi-head attention mechanisms. The copy mechanism (Copynet \cite{DBLP:conf/acl/GuLLL16} and Pointer-Generator \cite{DBLP:conf/acl/SeeLM17}) is proposed to incorporate the ability of copying word into the Seq2Seq framework, which enable the model to copy words from the source sequence. Recently, generative pretrained language model like  GPT-2\cite{radford2019language}, GPT-3\cite{brown2020language}, UNILM\cite{dong2019unified}, UNILMv2\cite{bao2020unilmv2}, BART\cite{lewis2020bart}, PALM\cite{bi2020palm} has dominate this area. The pre-training and fine-tuning paradigm has been successful in many areas. The pre-trained corpus and paradigm have been 
% proved to have a significant impact on the downstream tasks by \cite{zhang2020pegasus,gururangan2020don}.

% \subsection{Review Response Generation}

% Review response generation task has been studied for different application domain in recent year. \cite{gao2019automating} proposed a Neural Machine Translation (NMT)-based neural network which encodes user reviews and generate developer's responses for mobile apps. Although external review attributes including review length, rating, predicted sentiment, app category, and pre-defined keywords, are adopted to better encode the semantics of user reviews, their model don't use the information from current application itself. \cite{zhao2019review} propose a  Seq2Seq framework for the review response generation task in E-commerce platforms, which incorporates product information by a gated multi-source attention mechanism and a copy mechanism. \cite{zhao2019review} only use the product properties as external knowledge when encoding the source part, but we also including product title and historical responses for similar reviews as knowledge source, another challenge is that these multi-source information has different structure.

% \subsection{Retrieval-Augmented Generation}

% Recently, multiple works \cite{lee2019latent,DBLP:conf/icml/GuuLTPC20,karpukhin2020dense} pre-train neural knowledge retriever that retrieves knowledge from a textual knowledge corpus (e.g. Wikipedia), these pertained knowledge retriever fine-tuned get a SOTA result on  Open-domain Question Answering task. Our method also use a retriever to recall (review,response) pairs of similar reviews as textual knowledge. Due to the limited number of retrieval pool and the specificity of our task, we use a simple ranking model with ElasticSearch\cite{gormley2015elasticsearch} as a replacement rather than end2end retriever which is too expensive. \cite{DBLP:conf/eacl/IzacardG21} and \cite{DBLP:conf/nips/LewisPPPKGKLYR020} introduce retrieval augmented generative models for open domain question answering, Our approach differs from these works by how the generative model processes multi-source knowledge including text and structural product properties and how the generating process align each sub-sequence of user reviews.


% \section{Conclusion}
% In this work, we propose the concept of persuasive responses to user reviews in E-commerce. Such persuasive responses are beneficial to customer service providers. This area has not been noticed by past researchers. In order to solve the problem of the source of persuasiveness, we designed a multi-source encoder to encode information from different sources, including product title, seller name, product attributes, product historical (review, response) pairs, etc. In order to further improve the relevance of comments in the generation of persuasive responses, we designed HAM so that the model refers to different aspects when generating different words. In the persuasive response generation, both automatic evaluation and manual evaluation methods have proved our proposed method. exceeds the state of the art text generation model.

% %%
% %% The next two lines define the bibliography style to be used, and
% %% the bibliography file.
% \bibliographystyle{ACM-Reference-Format}
% \bibliography{sample-base}

% %%
% %% If your work has an appendix, this is the place to put it.
% % \appendix

% % \section{Research Methods}

% % \subsection{Part One}

% % Lorem ipsum dolor sit amet, consectetur adipiscing elit. Morbi
% % malesuada, quam in pulvinar varius, metus nunc fermentum urna, id
% % sollicitudin purus odio sit amet enim. Aliquam ullamcorper eu ipsum
% % vel mollis. Curabitur quis dictum nisl. Phasellus vel semper risus, et
% % lacinia dolor. Integer ultricies commodo sem nec semper.

% % \subsection{Part Two}

% % Etiam commodo feugiat nisl pulvinar pellentesque. Etiam auctor sodales
% % ligula, non varius nibh pulvinar semper. Suspendisse nec lectus non
% % ipsum convallis congue hendrerit vitae sapien. Donec at laoreet
% % eros. Vivamus non purus placerat, scelerisque diam eu, cursus
% % ante. Etiam aliquam tortor auctor efficitur mattis.

% % \section{Online Resources}

% % Nam id fermentum dui. Suspendisse sagittis tortor a nulla mollis, in
% % pulvinar ex pretium. Sed interdum orci quis metus euismod, et sagittis
% % enim maximus. Vestibulum gravida massa ut felis suscipit
% % congue. Quisque mattis elit a risus ultrices commodo venenatis eget
% % dui. Etiam sagittis eleifend elementum.

% % Nam interdum magna at lectus dignissim, ac dignissim lorem
% % rhoncus. Maecenas eu arcu ac neque placerat aliquam. Nunc pulvinar
% % massa et mattis lacinia.

% \end{document}
% \endinput
% %%
% %% End of file `sample-sigconf.tex'.

